Domain-independent Dominance of Adaptive Methods

From a simplified analysis of adaptive methods, we derive AvaGrad, a new optimizer which outperforms SGD on vision tasks when its adaptability is properly tuned. We observe that the power of our method is partially explained by a decoupling of learning rate and adaptability, greatly simplifying hyperparameter search. In light of this observation, we demonstrate that, against conventional wisdom, Adam can also outperform SGD on vision tasks, as long as the coupling between its learning rate and adaptability is taken into account. In practice, AvaGrad matches the best results, as measured by generalization accuracy, delivered by any existing optimizer (SGD or adaptive) across image classification (CIFAR, ImageNet) and character-level language modelling (Penn Treebank) tasks.

==> Makefile <==
# programs
PDFLATEX = pdflatex
CP       = cp
RM       = rm
GREP     = grep
DIFF     = diff -q
TOUCH    = touch

# input and output files
TEXFILE = avagrad_arxiv.tex
PDFFILE = avagrad_arxiv.pdf
TEXINCLUDES = $(wildcard include/*)

# intermediate files
TEXLOG     = $(basename $(TEXFILE)).log
AUXFILE    = $(basename $(TEXFILE)).aux
OUTFILE    = $(basename $(TEXFILE)).out
OLDAUXFILE = $(AUXFILE).old

# arxiv submission files
ARXIV_FILES := $(if $(wildcard files.txt),$(shell cat files.txt),)
ARXIV_OUT   := arxiv.tar.gz

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
.PHONY: pdf
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.
# Then PDFLaTeX is re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES)
	$(TOUCH) $(AUXFILE)
	$(CP) $(AUXFILE) $(OLDAUXFILE)
	$(PDFLATEX) $<
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# arxiv submission
.PHONY: submit
submit: $(ARXIV_OUT)
$(ARXIV_OUT): files.txt $(ARXIV_FILES)
	@COPYFILE_DISABLE=1 tar cvzfh $(ARXIV_OUT) $(ARXIV_FILES)

# This rule cleans out the files made by the make process.
.PHONY: clean
clean:
	$(RM) -f $(AUXFILE)\
                 $(OLDAUXFILE)\
                 $(OUTFILE)\
                 $(TEXLOG)\
                 $(PDFFILE)\
                 $(ARXIV_OUT)

